I'll Be Back: On the Multiple Lives of Users of a Mobile Activity Tracking Application

Mobile health applications that track activities, such as exercise, sleep, and diet, are becoming widely used. While these activity tracking applications have the potential to improve our health, user engagement and retention are critical factors for their success. However, long-term user engagement patterns in real-world activity tracking applications are not yet well understood. Here we study user engagement patterns within a mobile physical activity tracking application consisting of 115 million logged activities taken by over a million users over 31 months. Specifically, we show that over 75% of users return and re-engage with the application after prolonged periods of inactivity, no matter the duration of the inactivity. We find a surprising result that the re-engagement usage patterns resemble those of the start of the initial engagement period, rather than being a simple continuation of the end of the initial engagement period. This evidence points to a conceptual model of multiple lives of user engagement, extending the prevalent single life view of user activity. We demonstrate that these multiple lives occur because the users have a variety of different primary intents or goals for using the app. We find evidence for users being more likely to stop using the app once they achieved their primary intent or goal (e.g., weight loss). However, these users might return once their original intent resurfaces (e.g., wanting to lose newly gained weight). Based on insights developed in this work, including a marker of improved primary intent performance, our prediction models achieve 71% ROC AUC. Overall, our research has implications for modeling user re-engagement in health activity tracking applications and has consequences for how notifications, recommendations as well as gamification can be used to increase engagement.

==> 030data_old.tex <==
% !TEX root = paper-multiple-lives.tex


\subsection{User Demographics}
Maybe: We further show how multiple lives patterns vary with demographics. Figure~\ref{fig:lifetime_returning_prob_across_demographics}
\tim{ jure suggested skipping this section --- not in main focus --- fine to use for prediction. think about brief note}



% join time and demographics 
\begin{figure*}[t]
\begin{subfigure}{.245\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/demographics/scatter_join_time}
  \caption{}
     \label{fig:scatter_join_time}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/demographics/scatter_user_profile_age_cat}
  \caption{}
     \label{fig:scatter_age}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/demographics/scatter_user_profile_bmi_cat}
  \caption{}
     \label{fig:scatter_bmi}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/demographics/scatter_user_profile_gender}
  \caption{}
     \label{fig:scatter_gender}
\end{subfigure}
\caption{Lifetime and returning probability across demographic groups}
\label{fig:lifetime_returning_prob_across_demographics}
\end{figure*}










\subsection{Dataset Description}






\subsection{Definitions}
\subsubsection{Definition of Concepts}
\begin{itemize}
	\item \textbf{Inter-life gap $\delta$}: The user needs to have days without manual checkins to be declared ``Dead''. Unless otherwise specified, $\delta$ = 30 days is used in the paper.
	\item \textbf{Activities}: we are only focusing on ``manual activities'', i.e., activities that are not automatically logged.
	\item \textbf{Life}: We call a period without $\geq \delta$ days of manual check-in absence a ``life''; lifetime is calculated as the $T_{\text{last check-in}} - T_{\text{first check-in}}$ in this life.
	\item \textbf{Performance}: For some activities (e.g., running and weight logging), there are some values associated with the user's activity level or physical status such as running duration, or weight. In this paper, we generally refer such quantities as ``performance''.
\end{itemize}

\subsubsection{Definition of Summary Statistics}

When analyzing users' usage patterns, we focus on following summary statistics:

\begin{itemize}
	\item \textbf{Check-in frequency}: A measure of user's activeness, calculated as user Weekly check-in count.
	\item \textbf{Activity Entropy}: A measure of a user's activity diversity. It can be regarded as a combination of \textit{number of distinct activities} and \textit{portion of the most frequent activity}.
	\item \textbf{Persistence}: Weekly difference in Check-in frequency and activity diversity, indicating how much can the user keep up with his/her previous activity level. It is calculated as the average of inter-week difference.
\end{itemize}




==> 050multiple_lives_old.tex <==
% !TEX root = paper-multiple-lives.tex
Figure~\ref{fig:ccdf_number_of_lives_dist} shows many users have multiple lives regardless the choice of inter-life gap $\delta$. In this subsection, we will first examine how a user's single life look like, then zoom out to see how users reincarnate from ``death'' by coming back to the app again.

\subsection{Intra-Life Patterns}
Figure~\ref{fig:sliding_window} shows how check-in frequency and activity entropy look like in a single life. We see that for in every life a each lifetime group, users always start with high check-in frequency and activity entropy. As time goes on, users check in less and less frequently with lower diversity and eventually drop out from the app.

Users are also very concentrated: Figure~\ref{fig:number_of_activities_took_to_cover_x_checkins} suggest that most users' most check-ins are from one or a few activities.

Check-in frequency and activity entropy reflect two aspects of a user: his/her activeness and diversity level. How fast do those two metrics change indicates the persistence of the user.
Figure~\ref{fig:single_life_characteristic} shows that those summary statistics are  associated with for how long a user is going to live: generally, a longer term user tends to have higher level of check-in frequency and diversity as well as smaller weekly change in those values. Our prediction task later shows that those are indeed strong predictors for users' lifetime.

\begin{figure}[tb]
\begin{subfigure}{.5\textwidth}
  \includegraphics[width=\textwidth]{FIG/single_life/checkin_freq_sliding_window}
  \caption{}
     \label{fig:checkin_freq_sliding_window}
\end{subfigure}
\hfill

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/single_life/entropy_sliding_window}
  \caption{}
     \label{fig:entropy_sliding_window}
\end{subfigure}%

\caption{Weekly check-in count and activity entropy of different user lifetime groups} 
\label{fig:sliding_window}
\end{figure}



\begin{figure}[tb]
\begin{subfigure}{.23\textwidth}
  \includegraphics[width=\textwidth]{FIG/single_life/first_week_checkin}
  \caption{First week check-in count}
     \label{fig:first_week_checkin}
\end{subfigure}
\hfill
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/single_life/first_week_entropy}
  \caption{First week activity entropy}
     \label{fig:first_week_entropy}
\end{subfigure}
\vfill
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/single_life/weekly_checkin_derivative}
  \caption{Average weekly check-in count derivative}
     \label{fig:weekly_checkin_derivative}
\end{subfigure}
\hfill
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{FIG/single_life/entropy_derivative}
  \caption{Average weekly activity entropy derivative}
     \label{fig:entropy_derivative}
\end{subfigure}
\caption{Usage patterns of users from different lifetime group} 
\label{fig:single_life_characteristic}
\end{figure}


\subsection{Inter-Life Patterns}
Figure~\ref{fig:ccdf_number_of_lives_dist} already suggests many users come back after leaving the app, but the question unanswered is: why do they come back and do they come back as a different person?

\subsubsection{Why users comes back?}
Figure~\ref{fig:number_of_activities_took_to_cover_x_checkins} shows users often focus on a few activities. Hence, we look at several activities with measurable performance: weight, running, walking, and sleep report. Respectively, we examine  how the weight value, running duration, walking duration, and sleeping time change in each life.
The result is presented in figure~\ref{fig:zig_zag_plots}. As we can see, users comes in at lower performance level (heavier weight or shorter running duration for example) and leave with higher performance level (lighter weight or longer running duration, for example). However, when users come back, they on average come back at lower performance level than when they leave.



\subsubsection{Do users come back differently?}
Figure~\ref{fig:number_of_activities_took_to_cover_x_checkins} shows users are often concentrated on a few activities. This is also true across different lives: users tend to focus on the same primary activities as well (Figure~\ref{fig:same_most_freq_activity}). Even after the user leaves the app, there is a good chance that the user comes back and still focus on the very same activity.

On the other hands, users also come back differently. They come back refreshed. Even though users gradually become less engaged by having lower check-in frequency and entropy, Figure~\ref{fig:zig_zag_summary_stats} shows that when users come back, they come back with higher check-in frequency and entropy. In other words, a user come back differently as a more motivated person.


==> 060discussion_old.tex <==
\subsection{User Lifecycle and Reincarnation}
Following is our conceptual model explaining why users usually have multiple lives in using activity tracking app.

\subsubsection{Users Join with a Purpose}
Figure~\ref{fig:users_are_concentrated}: users mostly concentrated on a few activities and users' primary activities often do not change often. Along with Figure~\ref{fig:most_freq_activity_vs_lifetime_vs_prob_of_coming_back}, it suggest the primary activity could be predictive of user return rate.

\subsubsection{Users Start Motivated and Gradually Become Less Diverse and Frequent}
Figure~\ref{fig:sliding_window}: Users become less frequent and less diverse overtime

\subsubsection{Users Leave When Their Goals are Fulfilled}
Figure~\ref{fig:zig_zag_plots}: users join when weight is high, running duration is low, etc. and leave with some improvements. It suggests users join with a purpose in mind (e.g., to lose weight or run for longer duration), and leave when the goal is fulfilled.

\subsubsection{Users Come Back When They Need It Again}
For those who come back, they either did not fulfill the goal in their previous life or fell back to their their previous (or worse) activity level after leaving the app, which results in such zig-zag lines.
Users come back re-motivated (Figure~\ref{fig:zig_zag_summary_stats}).

\subsection{Implication of Increasing User Engagement in a Multiple-Life Paradigm}
What can the app developer do to increase user engagement and returning rate? We believe our research has shed some light on this.

\subsubsection{Identify short-term from long-term users}
As the following experiments section will show, we are able to identify short-term user vs. longer-term user. Hence the app developer could target short-term users to improve their engagement and try to convert them into longer term users.

\subsubsection{Identify loyal activities and app improvement direction}
Figure~\ref{fig:most_freq_activity_vs_lifetime_vs_prob_of_coming_back} in Latex doc shows that users with different primary activities are related to different level of lifetime and returning probability after leave. Hence, the app developer could either conduct campaigns to keep users with primary activities that are with both high return rate and long lifetime (top-right activities in Figure~\ref{fig:most_freq_activity_vs_lifetime_vs_prob_of_coming_back}) or try to focus on improving features associated with low return rate and short lifetime (bottom-left activities in Figure~\ref{fig:most_freq_activity_vs_lifetime_vs_prob_of_coming_back}).

\subsubsection{Bring users back} Figure 5 suggest users who come back are either did not improve much during their last life or have reverted their improvement after leaving the app. So the app developer could target users who did not change much during the app usage or send push notifications asking if the user wan to improve again. Note that along with other features.

\subsection{Identifying Users with Long Lifetime}
They are several factors that contribute to for how long a user will keep using this activity tracking app.

\subsubsection{Performance Change}
If the user has improved or not in terms activities he/she does. We use weight, running duration, walking duration, and sleeping time as performance metrics as they are relatively popular activities in the app with measurable performance change.

\subsubsection{Usage Pattern}
Figure~\ref{fig:single_life_characteristic} shows long-term users tend to be more active (Figure~\ref{fig:first_week_checkin}, higher check-in frequency), more diverse (Figure~\ref{fig:first_week_entropy}, higher entropy), and more persistent (Figure~\ref{fig:weekly_checkin_derivative}~\ref{fig:entropy_derivative}, smaller derivative) 

\subsubsection{Primary Activity}
Figure~\ref{fig:most_freq_activity_vs_lifetime_vs_prob_of_coming_back} suggests users with different primary activities have differently expected lifetime and returning rate. Top right activities are ones often associated with loyal users, who live longer and come back more often, while bottom left activities 

\subsubsection{Join Time and Demographics}
Figure~\ref{fig:lifetime_across_demographics} shows early joiners generally live longer. However, for early joiners' early lives, when the app was less well-refined, they may have shorter lives. Different BMI, age, and gender also play roles in identifying long-term users.


\subsection{Identifying Users Who Will Come Back}
We also look into what kinds of users will be more likely to come back. This is an inherently harder problem as there could be factors influencing a user's return rate during the user's absent period, which we do not observe. Despite such difficulty, there are still observable features during a user's current life that are useful in predicting user returning probability.

\subsubsection{Lifetime of current life}
Figure~\ref{fig:lifetime_vs_prob_coming_back}: For first life (blue line) medium lifetime is correlated with higher retention. For later lives short lives often related to more lives.\\
Interpretation: Those who join and leave quickly usually don't come back. Short lives later don’t mean the same thing, they are more likely to come back again. As for long lives, usually they have a more fruitful life and when they leave, they leave for good.
Figure~\ref{fig:lifetime_dist}: Lifetime gets shorter and shorter in later lives;\\

\subsubsection{Primary Activity}
Figure~\ref{fig:most_freq_activity_vs_lifetime_vs_prob_of_coming_back}: Users with different primary activities have different average lifetime and return probability.
What can Bojan do: either conduct campaign to bring back loyal users (top right), or to improve the app to engage users with less-loyal primary features (drink, food, cardio)

\subsubsection{Performance Change}
Even though Figure~\ref{fig:zig_zag_plots} suggests a user come back when he/she need it again, it is hard to tell what happens to the user when he/she is not using the app. Hence, even though performance change has some predictive power on user's returning probability (Figure~\ref{fig:lifetime_prediction_feature_comparison}), it is a less useful feature than it is in determining a user's lifetime.

\subsubsection{Join Time and Demographics}
Figure~\ref{fig:return_prob_across_demographics} shows join time and demographics also matter.


==> 070experiments_old.tex <==
% !TEX root = paper-multiple-lives.tex

% \subsection{Lifetime Prediction}
% Figure~\ref{fig:lifetime_prediction_feature_comparison}

% Features: first week checkin count, first week diversity, first 4 weeks checkin count derivative, first 4 weeks diversity derivative, most frequent activity in first 4 weeks, join time, demographics

% \begin{figure}[tb]

% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{FIG/lifetime_prediction_feature_comparison}
%   \caption{Feature Comparison}
%      \label{fig:lifetime_prediction_feature_comparison}
% \end{subfigure}
% \vfill
% \begin{subfigure}{.45\textwidth}
%   \includegraphics[width=\textwidth]{FIG/lifetime_prediction}
%   \caption{Performance with varying $w_1$ and $w_2$}
%      \label{fig:lifetime_prediction}
% \end{subfigure}

% \caption{After observing first 4 weeks, predict if a user is going to leave in the next $w_1$ days or is going to live longer than $w_2$ days. 10-fold cross validation is used.} 
% \label{fig:lifetime_prediction_feature_comparison}
% \end{figure}



% \subsection{User Return Prediction}
% Figure~\ref{fig:come_back_prediction_feature_comparison}

% Features: Lifetime in current life, most frequent activity in first 4 weeks, performance (w.r.t. weight, running/walking/sleeping duration) change percentage, join time, demographics

% \begin{figure}[tb]
% \centering
% \includegraphics[width=0.48\textwidth]{FIG/come_back_prediction_feature_comparison}
% \caption{Predict if a user will come back after each life. 10-fold cross validation is used.}
% \label{fig:come_back_prediction_feature_comparison}
% \end{figure}

==> Makefile <==
RCSFLAGS= -l
MAIN=paper-multiple-lives
TEXPARTS= \
	000abstract.tex		\
	010intro.tex		\
	020related.tex		\
	030single_life.tex	\
	040multiple_lives.tex	\
	050demographics.tex \
	060experiments.tex \
	070conclusion.tex

BIBPARTS= *.bib
LPR = pspr # or change to 'qpr -q ps3'
POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
FIGPARTS = FIG

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS)
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

try: $(MAIN).tex
	pdflatex $(MAIN)

print: $(MAIN).ps
	$(LPR) $(MAIN).ps

checkout:
	cvs checkout $(RCSFLAGS) $(MAIN).tex $(TEXPARTS)

checkin:
	cvs checkin $(RCSFLAGS) -f $(MAIN).tex $(TEXPARTS)

clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.blg *.fdb_latexmk *.fls *.synctex.gz *.log *.blg *.toc all.tar* uu *~ *.bak *.out $(MAIN).pdf

spotless: clean
	\rm -f $(MAIN).ps

all.tar:
	tar cvfh all.tar makefile $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) README

uu: all.tar
	gzip all.tar
	uuencode all.tar.gz all.tar.gz > uu

bundle.all: $(TEXPARTS) 
	bundle  README $(TEXPARTS) $(BIBPARTS) makefile > bundle.all

zip:
	cmd /C "pkzip $(MAIN).zip -P $(MAIN).pdf Makefile *.cls *.tex *.bib FIG/*.eps"

